Implicit Affordance Acquisition via Causal Action-Effect Modeling in the Video Domain

Affordance knowledge is a fundamental aspect of commonsense knowledge. Recent findings indicate that world knowledge emerges through large-scale self-supervised pretraining, motivating our exploration of acquiring affordance knowledge from the visual domain. To this end, we augment an existing instructional video resource to create the new Causal Action-Effect (CAE) dataset and design two novel pretraining tasks -- Masked Action Modeling (MAM) and Masked Effect Modeling (MEM) -- promoting the acquisition of two affordance properties in models: behavior and entity equivalence, respectively. We empirically demonstrate the effectiveness of our proposed methods in learning affordance properties. Furthermore, we show that a model pretrained on both tasks outperforms a strong image-based visual-linguistic foundation model (FLAVA) as well as pure linguistic models on a zero-shot physical reasoning probing task.

==> sections/affordances_preamble.tex <==
% task/resource/dataset name
\newacronym{cae}{CAE\xspace}{Causal Action-- Effect}
\newacronym{vl}{VL\xspace}{visual--linguistic}
\newacronym{prost}{PROST\xspace}{Physical Reasoning about Objects through Space and Time}

% our task-specific name
\newacronym{multi}{MULTI-CAE\xspace}{Multi-task on Causal Action--Effect Modeling}
\newacronym{mam}{MAM\xspace}{Masked Action Modeling}
\newacronym{mem}{MEM\xspace}{Masked Effect Modeling}
\newacronym{map}{MAP\xspace}{Masked Action Prediction}
\newacronym{mep}{MEP\xspace}{Masked Effect Prediction}

% model name
\newcommand{\mamVTten}{\textsc{MAM-VL-10PER}\xspace}
\newcommand{\mamVTtenrandom}{\textsc{MAM-VL-10PER-Rnd}\xspace}

\newcommand{\mamVT}{\textsc{MAM-VL}\xspace} % FULL
\newcommand{\mamVTrandom}{\textsc{MAM-VL-Rnd}\xspace} % FULL

\newcommand{\mamT}{\textsc{MAM-L}\xspace} % FULL
\newcommand{\mamTrandom}{\textsc{MAM-L-Rnd}\xspace} % FULL

\newcommand{\mamVTrandomTnoAFT}{\textsc{MAM-VL-Rnd-NO-AFT}\xspace} % FULL

\newcommand{\memVTten}{\textsc{MEM-VL-10PER}\xspace}
\newcommand{\memVTtenrandom}{\textsc{MEM-VL-10PER-Rnd}\xspace}

\newcommand{\memVT}{\textsc{MEM-VL}\xspace} % FULL
\newcommand{\memVTrandom}{\textsc{MEM-VL-Rnd}\xspace} % FULL

\newcommand{\memV}{\textsc{MEM-V}\xspace} % FULL
\newcommand{\memVrandom}{\textsc{MEM-V-Rnd}\xspace} % FULL

\newcommand{\multiVT}{\textsc{Multi-CAE-VL}\xspace}
\newcommand{\multiT}{\textsc{Multi-CAE-L}\xspace}
\newcommand{\multiV}{\textsc{Multi-CAE-V}\xspace}
\newcommand{\multiVTrandom}{\textsc{Multi-CAE-VL-Rnd}\xspace}

\newcommand{\roberta}{RoBERTa-B\xspace}

% Added by Carina
\newcommand{\words}[1]{``#1''\xspace}
\newcommand{\word}[1]{``#1''\xspace}
\newcommand{\object}[1]{\textsl{#1}\xspace}
